DeceptPrompt: Exploiting LLM-driven Code Generation via Adversarial Natural Language Instructions

With the advancement of Large Language Models (LLMs), significant progress has been made in code generation, enabling LLMs to transform natural language into programming code. These Code LLMs have been widely accepted by massive users and organizations. However, a dangerous nature is hidden in the code, which is the existence of fatal vulnerabilities. While some LLM providers have attempted to address these issues by aligning with human guidance, these efforts fall short of making Code LLMs practical and robust. Without a deep understanding of the performance of the LLMs under the practical worst cases, it would be concerning to apply them to various real-world applications. In this paper, we answer the critical issue: Are existing Code LLMs immune to generating vulnerable code? If not, what is the possible maximum severity of this issue in practical deployment scenarios? In this paper, we introduce DeceptPrompt, a novel algorithm that can generate adversarial natural language instructions that drive the Code LLMs to generate functionality correct code with vulnerabilities. DeceptPrompt is achieved through a systematic evolution-based algorithm with a fine grain loss design. The unique advantage of DeceptPrompt enables us to find natural prefix/suffix with totally benign and non-directional semantic meaning, meanwhile, having great power in inducing the Code LLMs to generate vulnerable code. This feature can enable us to conduct the almost-worstcase red-teaming on these LLMs in a real scenario, where users are using natural language. Our extensive experiments and analyses on DeceptPrompt not only validate the effectiveness of our approach but also shed light on the huge weakness of LLMs in the code generation task. When applying the optimized prefix/suffix, the attack success rate (ASR) will improve by average 50% compared with no prefix/suffix applying.

==> intro.tex <==
%-------------------------------------------------------------------------------
\section{Introduction}
%-------------------------------------------------------------------------------
\chaowei{LLM has been used in many applications, ranging from XXX. .... One important ability of current LLMs is the code ability ... why code is important ... it has been used in many safety-critical applications Thus, it is  important to understand safety ...  } 
Large Language Models (LLMs), trained on extensive corpora, have garnered significant attention due to their remarkable capabilities and adaptability across various tasks~\cite{}.
Moreover, numerous applications have been developed that rely on or incorporate these LLMs~\cite{}.
% LLM for code tasks
LLMs designed for code generation hold great promise in expediting software development~\cite{}. 
% poor performance and the essential properties of the code 
However, when employing such generated code, two crucial considerations come to the forefront: 1) the code's functionality and 2) its security.
While code generated by LLMs can be aligned with desired functionality through training on extensive corpora, the presence of numerous security vulnerabilities within these large training datasets~\cite{} (such as those from GitHub repositories~\cite{}) significantly compromises the security of the resulting code. Consequently, LLMs often produce code that is highly susceptible to vulnerabilities. This not only obstructs the practical utilization of these applications but also amplifies the dissemination of insecure code, potentially leading to severe consequences and threats to software and societal progress~\cite{}.


% efforts of alignment on functionality
\chaowei{No need this paragraph}
Although model providers and companies have employed human alignments~\cite{} in an attempt to align LLM outputs, these efforts still fall short of consistently producing secure code suitable for real-world applications~\cite{}. The majority of alignment methods primarily concentrate on ensuring that models do not generate malicious code~\cite{} and improving the functionality of the generated code~\cite{}.

% recently work on attack llms consider functionality instead of vulnerability
\chaowei{To understand xxx, a standard way is to red-team the LLMs by generating adversarial examples.... Discussing how existing work generate adversarial examples. However, such methods does not consider the core property of code : xxx and xxx. Explain why XXX and XXX is important by giving some examples.   }
Recent efforts aimed at attacking LLMs have largely concentrated on adversarial attacks within specific code-related tasks~\cite{}, such as code classification~\cite{} and code summarization~\cite{}. These approaches utilize adversarial code snippets, painstakingly crafted to serve as LLMs inputs, with the goal of tricking the models into generating incorrect results. The objective of such attacks is to expose the weaknesses of the abilities of LLMs on related task instead of security issues, which aim at leading LLMs to produce responses with wrong functionality. For instance, in~\cite{}, adversarial code examples are employed to induce LLMs to make wrong classifications, while in~\cite{}, the focus is on attack LLMs on code translation tasks. In these scenarios, LLMs are typically tasked with processing the code input rather than generating code solely based on natural language prompts, and the attack aim is to modify the functionality of the generated output.

 
% works study the security issues of code generation not the functionality
However, vulnerabilities present in generated code have not received the same level of attention as the reliable functionality of LLMs themselves. Only a handful of studies have paid attention to the vulnerabilities in code produced by LLMs within code generation schemes~\cite{}. Notably, \cite{} has established a benchmark and developing an automated method to evaluate security issues in code generated by LLMs.
Some efforts, like those in \cite{}, have explored the use of soft prefixes to regulate the generation of code, controlling the vulnerability and security of the generated code while preserving functionality. 
Nevertheless, these approaches either 
only focus on on evaluating security of the completed code where the given prompt is usually the former part code with inflexible natural language comments without further considering the deep mechanism of natural language prompts impact on the security of the generated code, 
or they rely on soft prompts to steer the generation process while potentially sacrificing semantics of the prompt.
In a recently more practical scheme, programmers and everyday users who engage in coding typically prefer to employ pure natural language descriptions with semantics, especially when they lack a precise vision of the target code. Surprisingly, no prior work has undertaken the consideration of what is arguably the most practical and significant  scheme: Can we will pure semantic natural language prompts to impact the security of generated code?

% our target
This leads to an further important question: Can we develop an attack framework to evaluate the LLMs code generation process by  targeting the code output to specific vulnerability without affecting its functionality?
To bridge this gap, this study undertakes a comprehensive exploration in this new code generation attack scheme. 
We introduce a novel attack framework that aims to attack LLMs for code generation tasks using additional semantic natural language prompts (\texttt{prefix}/\texttt{suffix}). Our objective is to compel LLMs to generate code that maintains its functionality while incorporating specified vulnerabilities.

% insight or challenge
\subsection{Challenges}
To develop and design a practical attack for code generation LLMs, we should simultaneously consider three main essential challenges: 1) how to preserve the functionality of the output coded, 2) how to target the code with specific vulnerabilities? and 3) how to preserve the semantics of the natural language \allfix?
\paragraph{Challenge I: Functionality Preservation.}
Due to the diversity of the natural language prompts and the diverse training corpus, change a single word in the input prompt may lead to the difference in functionality of the generated output~\cite{} from the LLMs. Besides that, the context environment of a chat-style\cite{} (the most popular mode for using LLMs) LLM process may impact the results from LLMs, e.g., the information in the history record may be used by LLMs to generate the answers~\cite{}. More importantly, due to the diversity of code forms~\cite{}, the solutions to the same question can various~\cite{}, and also the limitations for LLMs' capability to generate totally consistent output, it is hard to ensure the changes of forms will not impact the functionality.
\paragraph{Challenge II: Target Vulnerability Injection.}
One key challenge is how to inject the target or desired vulnerability in the original output. Basically, the generated codes may have vulnerabilities due to super weak or almost no alignment on the code security aspect, how to target the output to the specific vulnerabilities or improve the probability of generating target vulnerability from all potential existed vulnerabilities is the key challenge. Moreover, due to the diversity of the code forms, the locations of the vulnerabilities is various, which will increase the difficulty for the vulnerability injection.
\paragraph{Challenge III: Preservation of Natural Language Prompt Semantics.}
When attacking Code LLMs, especially in a chat-style context, maintaining the semantics of the input \allfix is of paramount importance. Soft prompts~\cite{} generated through gradients can be easily detected by perplexity-check tools~\cite{}. In contrast, prompts with preserved semantics are more practical and reasonable to be used for attack. Ensuring that the prompts remain meaningful without any indications of vulnerability is a pivotal aspect of the attack framework.




\subsection{Proposed Solution}
To tackle the aforementioned challenges, we introduce \system, a novel framework that leverages genetic algorithms and a unique split control loss. Our approach begins by creating an additional \texttt{prefix/suffix} serving as a template seed. The template prompt consists of benign, semantically meaningful context that avoids any vulnerability-related information or indicators. Importantly, it has no impact on the objective of the generation task, e.g., ``My grandmother is eager to learn this method, can you assist her?''\footnote{This example is a simplified representation of the prefix and suffix types, and real cases are typically more detailed and extensive.} Subsequently, we generate a series of prompts based on this seed prompt, ensuring that the underlying semantics remain unaltered.



\textbf{Semantic Preserving Evolution.} Upon generating this set of prompts, our next step involves optimizing the \allfix to increase the probability of generating the code with target vulnerabilities. To maintain the semantics of the natural language prompt, we depart from the conventional gradient-based optimization~\cite{} and, instead, employ genetic algorithms (GA)~\cite{}. This choice ensures that we keep the semantics of the optimization targets.
In our approach, each prompt in the group of generated \allfix is treated as a ``gene'', and we apply ``Crossover'' and ``Mutation'' to the selected elites. ``Crossover'' involves exchanging the inner sentences between the chosen sentences, while ``Mutation'' entails querying ChatGPT~\cite{} to paraphrase the sentence without altering its semantics. Furthermore, we maintain a comprehensive global word ranking library, allowing us to substitute synonyms with higher-ranked alternatives based on the optimization loss.



\textbf{Fine Grained Loss.} We have meticulously design the optimization process for our attack framework to address the dual objectives of maintaining code functionality and precisely introducing specific vulnerabilities into the output code. To achieve this, we initiate by defining a target code that is both functionally correct and includes the specific vulnerability.
A key insight lies in the recognition of two distinct code categories from a security standpoint~\cite{}. The first category comprises ``benign'' code, free from vulnerabilities, while the second category encompasses ``vulnerable'' code, which serves as the root cause of vulnerabilities.
Thus, we divide the target code into several code snippets, categorizing them as either ``benign'' or ``vulnerable''. Subsequently, we calculate the loss independently as two different items. For the benign portion, the loss is to control the functionality of the generated code, ensuring it aligns with the intended function. Meanwhile, for the vulnerable code snippets, the loss is to guide the generated code to targeted with specific vulnerabilities. This precise loss design accelerates the optimization process, preserving functionality while pinpointing specific vulnerability directions.
To minimize the loss deviation between the target code and the generated one, we adopt a two-step approach. Firstly, we employ a greedy search to query the LLMs and obtain a solution code. Next, we manually inject the specific vulnerability we wish to target into the solution code, all the while ensuring that functionality remains unchanged.







\textbf{Evaluation.} To comprehensive evaluate and analyze the performance of \system, we constructed a dataset covering 25 different CWE types~\cite{} from~\cite{} and~\cite{} and, we also self manually constructed cases. We attack the most popular and recent Code LLMs including Code Llama~\cite{}, StarCoder~\cite{}, and WizardCoder~\cite{}. The size of the evaluated model varies from 3B to 15B. The results showcase the superior performance, and it successful attack all listed the Code LLMs with high attack success rate (ASR).

\subsection{Main contribution}
% research qusetion & contribution
We summarize our contribution as follows:
\begin{itemize}
    \item To the best of our knowledge, \system is the pioneering framework for target attacks on LLMs code generation task, augmenting benign semantic natural language context while ensuring specific vulnerability in the target output.
    \item We present a novel approach to maintaining the semantic integrity of \allfix during optimization process, employing multi-level transformations to expedite optimization.
    \item Our experiments uncover huge weakness in recent Code LLMs, revealing their susceptibility to semantic natural language inputs, even in the absence of explicit vulnerability cues.
    \item We have introduced a novel split-loss design for precise vulnerability injection, significantly enhancing optimization while preserving functionality.
    \item We construsct a brand new benchmark for target attacks on LLMs code generation task.
    \item A comprehensive analysis, including 25 different CWE types and model configurations, demonstrates the effectiveness of our approach.
\end{itemize}


==> tables/detailed_cwe.tex <==
\begin{table}[t]
\small
\caption{The classfication of CWEs for the case in our dataset.}
  \label{tab:cwe}
  \setlength{\tabcolsep}{1pt}
  \centering
  \begin{tabular}{| c | c | c |}
    \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
    {CWE} &  {Description} & Type \\
    \hline
    {CWE-20} & \small{Improper Input Validation} & \small{Missing Error} \\
    {CWE-22} & \small{Path Traversal }&  \small{Missing Error}\\
    {CWE-78} & \small{OS Command Injection} &  \small{Missing Error} \\
    {CWE-89} & \small{SQL Injection} &  Missing Error\\
    {CWE-119} & \small{Buffer Overflow} & Wrong Usage \\
    {CWE-125} & \small{Out-of-bound Read} & Missing Error\\
    {CWE-190} & \small{Integer Overflow} & Wrong Usage\\
    {CWE-200} & \small{Exposure of Sensitive Information} & Wrong Usage \\
    {CWE-250} & \small{Execution with Unnecessary Privileges} & Missing Error\\
    {CWE-259} & \small{Use of Hard-coded Password} & Wrong Usage \\
    {CWE-269} & \small{Improper Privilege Management} & Missing Error \\
    {CWE-295} & \small{Improper Certificate Validation} & Wrong Usage\\
    {CWE-327} & \small{Risky Cryptographic Algorithm} & Wrong Usage \\
    {CWE-330} & \small{Predictable IV with CBC Mode} & Wrong Usage \\
    {CWE-339} & \small{Small Seed Space in PRNG} & Wrong Usage \\
    {CWE-347} & \small{Improper Verification of Signature} &Wrong Usage\\
    {CWE-416} & \small{Use After Free} & Wrong Usage \\
    {CWE-476} & \small{NULL Pointer}  & Missing Error \\
    {CWE-477} & \small{Use of Obsolete Function}& Wrong Usage \\
    {CWE-502} & \small{Deserialization of Untrusted Data} & Missing Error\\
    {CWE-732} & \small{Incorrect Permission Assignment} & Wrong Usage \\
    {CWE-760} & \small{One-Way Hash with a Predictable Salt}& Wrong Usage\\
    {CWE-787} & \small{Out-of-Bound Write} & Wrong Usage \\
    {CWE-835} & \small{Infinite Loop} & Wrong Usage \\
    {CWE-1204} & \small{Weak Initialization Vector} & Wrong Usage\\
    \noalign{\global\arrayrulewidth1pt}\hline\noalign{\global\arrayrulewidth0.4pt}
  \end{tabular}
\end{table}





